Sparsistency of $\ell_1$-Regularized $M$-Estimators

We consider the model selection consistency or sparsistency of a broad set of $\ell_1$-regularized $M$-estimators for linear and non-linear statistical models in a unified fashion. For this purpose, we propose the local structured smoothness condition (LSSC) on the loss function. We provide a general result giving deterministic sufficient conditions for sparsistency in terms of the regularization parameter, ambient dimension, sparsity level, and number of measurements. We show that several important statistical models have $M$-estimators that indeed satisfy the LSSC, and as a result, the sparsistency guarantees for the corresponding $\ell_1$-regularized $M$-estimators can be derived as simple applications of our main theorem.

==> sections/assumpt.tex <==


%\textbf{Beta-min condition: } Let $\beta_{\min} = \min \left\{ \left\vert ( \beta^*)_k \right\vert: ( \beta^* )_k \neq 0 \right\} \geq \beta_{\min}$.  This is the so-called beta-min condition in \cite{Buhlmann2011} and is necessary in the proofs in \cite{Wainwright2009,Ravikumar2011}.

% \textbf{Bounded diagonal element: } The diagonal elements of $\nabla^2 L_n( \beta^* )$ satisfy $\left[ \nabla^2 L_n( \beta^* ) \right]_{i,i} \leq \sigma^2$ with some $\sigma > 0$ for all $i \in \{ 1, \ldots, p \}$. 



%\begin{rem}
%The local smoothness and local strong convexity conditions are equivalent to saying that 
%\begin{equation}
%\mu I \leq \left[ D^2 L_n ( \beta^* + \delta ) \right]_{\mathcal{S}, \mathcal{S}} \leq L I \label{eq_local_RIP}
%\end{equation}
%for $\delta$ small enough. This is closely related to but in general \emph{weaker} than the restricted isometry property (RIP), as we only require the the RIP condition (\ref{eq_local_RIP}) to hold \emph{locally}. In the linear model, since the $D^2 L_n$ is a constant, our local smoothness and local strong convexity conditions become exactly the RIP condition.
%\end{rem}

==> sections/exmp.tex <==
Now we show that some well-known self-concordant functions are also LUSC, and they satisfy the margin condition.

\begin{exmp}
It is easy to verify that the function $f( x ) = x - \ln x$ is $( x, \mathcal{N}_x )$-LUSC with parameter $ 2 ( 1 + \kappa^{-1} )^3 $ for any given $x \in \mathrm{dom}\, f = ( 0, \infty )$, where $$\mathcal{N}_x := \left\{ x + \delta: \left\vert \delta \right\vert \leq \frac{ x }{( 1 + \kappa )}  \right\}$$ with some $\kappa > 0$. Moreover, $f$ is $(x, \mathcal{F}_x)$-locally strong convex with $\mu = ( 1/4 ) x^{-2}$ with $$\mathcal{F}_x := \{ x + \delta: \left\vert \delta \right\vert \leq x \},$$ since for all $\delta$ such that $ x + \delta \in \mathcal{F}_x$, we have
\begin{equation}
\nabla^2 f( x + \delta ) = \frac{1}{\left( x + \delta \right)^2} \geq \frac{1}{\left( 2 x \right)^2}. \notag
\end{equation}

(Should replace all $x$ by $\beta$... Perhaps I should replace all $\beta$ in this paper by $\theta$...)
\end{exmp}

\begin{exmp} \label{exmp_loglinear}
We show that the function $f( \beta ) = \left\langle x, \beta \right\rangle - \ln \left\langle x, \beta \right\rangle$ with some $x \in \mathbb{R}^p$ is LUSC everywhere on $\mathrm{dom}\, f = \left\{ \beta: \left\langle x, \beta \right\rangle > 0 \right\}$.

Define $$r := \frac{\left\langle x, \delta \right\rangle}{\left\langle x, \beta \right\rangle}.$$ Suppose now that $\left\vert r \right\vert \leq ( 1 + \kappa )^{-1}$ with some $\kappa > 0$. Then we have
\begin{equation}
\frac{\left\vert D^3 f( \beta + \delta ) [ u, u, u ] \right\vert}{\left( D^2 f( \beta ) [u, u] \right)^{3/2}} = \frac{2}{\left\vert 1 + r \right\vert^3} \leq \frac{2}{( 1 - \left\vert r \right\vert )^3} \leq 2 \left( 1 + \kappa^{-1} \right)^3 \notag
\end{equation}
for any $\beta \in \mathrm{dom}\, f$, $\delta$ such that $x + \delta \in \mathrm{dom}\, f$, and any $u \in \mathbb{R}^p$. In order to ensure that $\left\vert r \right\vert \leq ( 1 + \kappa )^{-1}$, it suffices to require that
\begin{equation}
\left\Vert \delta \right\Vert \leq \frac{\left\langle x, \beta \right\rangle}{( 1 + \kappa ) \left\Vert x \right\Vert^* } \notag
\end{equation}
by H\"{o}lder's inequality, where $\left\Vert \cdot \right\Vert$ is a norm on $\mathbb{R}^p$ and $\left\Vert \cdot \right\Vert^*$ is the corresponding dual norm. Note that $\left\vert r \right\vert < 1$, so $\beta + \delta$ is always in $\mathrm{dom}\, f$.

Therefore $f$ is $( \beta, \mathcal{N}_\beta )$-LUSC with parameter $2( 1 + \kappa^{-1} )^3$ everywhere on $\mathrm{dom}\, f$, where 
\begin{equation}
\mathcal{N}_\beta := \left\{ \beta + \delta: \left\Vert \delta \right\Vert \leq \frac{\left\langle x, \beta \right\rangle}{( 1 + \kappa ) \left\Vert x \right\Vert^* } \right\} \notag
\end{equation}
with some constant $\kappa > 0$.

Moreover, $f$ is $( \beta, \mathcal{F}_\beta )$-locally strongly convex with parameter $\mu = ( 1 / 4 ) \lambda_{\min}$, where $$ \mathcal{F}_x := \left\{ \left\Vert \delta \right\Vert \leq \frac{\left\langle x, \beta \right\rangle}{\left\Vert x \right\Vert^*} \right\}, $$ and $\lambda_{\min}$ denotes the smallest eigenvalue of $\nabla^2 f( \beta )$, assuming $\lambda_{\min} > 0$, since for all $\delta$ such that $\beta + \delta \in \mathcal{F}_{\beta}$, we have
\begin{equation}
\nabla^2 f ( \beta + \delta ) = \frac{1}{\left( 1 + r \right)^2} \nabla^2 f( \beta ) \geq \frac{1}{4} \nabla^2 f( \beta ) \geq \frac{1}{4} \lambda_{\min} I. \notag
\end{equation}
\end{exmp}

\begin{exmp}
We show that the function $f( X ) = - \ln \det X$ defined on $\mathrm{dom}\, f = \left\{ X: X > 0, X \in \mathbb{R}^{p \times p} \right\}$ is both LUSC and locally strongly convex.

Let $U \in \mathrm{R}^{p \times p}$. We have
\begin{align}
D^3 f( X ) [ U, U, U ] &= - 2 \mathrm{Tr}\, \left[ \left( X^{-1/2} U X^{-1/2} \right)^3 \right], \notag \\
D^2 f( X ) [ U, U ]     &= \mathrm{Tr}\, \left[ \left( X^{-1/2} U X^{-1/2} \right)^2 \right]. \notag
\end{align}
Then, for all $X + \Delta \in \mathcal{F}_{X} := \left\{ X + \Delta: 0 < X + \Delta \leq X \ \right\}$, we have
\begin{equation}
D^2 f( X + \Delta )[ U, U ] \geq D^2 f( X )[ U, U ], \notag
\end{equation}
and, for all $X + \Delta \in \mathcal{N}_X := \mathcal{F}_X$, we have
\begin{equation}
\frac{\left\vert D^3 f ( X + \Delta )[ U, U, U ] \right\vert}{\left( D^2 f ( X )[ U, U ] \right)^{3/2}} \geq \frac{\left\vert D^3 f ( X )[ U, U, U ] \right\vert}{\left( D^2 f ( X )[ U, U ] \right)^{3/2}} = 2. \notag
\end{equation}

(I have not verified rigorously. And I have to also prove that $\mathcal{F}_X = \mathcal{N}_X$ is convex.)
\end{exmp}

==> sections/intro.tex <==
\vcmargin{This reads more like an introduction.}
\yhmargin{Motivation for model selection is lacking.}
%We consider a general statistical setting, where we are given $n$ independent samples drawn from some distribution $\mathbb{P}$ with a sparse parameter $\beta^* := \beta(\mathbb{P}) \in \mathbb{R}^p$. By sparse, we mean only $s$ entries of  $\beta^*$ are non-zero and $s\ll p$. We are interested in estimating the unknown parameter $\beta^*$ given the $n$ samples via the general class of $\ell_1$-regularized $M$-estimators that have the form:
%\begin{equation}
%\hat{\beta}_n := \arg \min_{\beta \in \mathbb{R}^p} L_n( \beta ) + \tau_n \left\Vert \beta \right\Vert_1, \label{eq_betahat}
%\end{equation}
%where $L_n$ is some convex function of the parameter $\beta$, and $\tau_n$ is a positive constant.

We consider a general statistical setting, where we are given $n$ independent samples that are statistically related to a sparse parameter $\beta^* \in \mathbb{R}^p$. By being sparse, we mean only $s$ entries of  $\beta^*$ are non-zero and $s\leq p$. We are interested in estimating the unknown parameter $\beta^*$ given the $n$ samples via the general class of $\ell_1$-regularized $M$-estimators that have the form:
\begin{equation}
\hat{\beta}_n := \arg \min_{\beta \in \mathbb{R}^p} L_n( \beta ) + \tau_n \left\Vert \beta \right\Vert_1, \label{eq_betahat}
\end{equation}
where $L_n$ is some convex function of $\beta$, and $\tau_n$ is a positive constant.

The formulation above addresses a broad range of applications in machine learning. A basic example is the sparse linear regression, where our goal is to estimate the sparse parameter $\beta^* \in \mathbb{R}^p$ given $\left\{ ( x_i, y_i ) \right\}_{i \in \{ 1, \ldots, n \}} \subset \mathbb{R}^p \times \mathbb{R}$. The vectors $x_1, \ldots, x_n$ are fixed, and the real numbers $y_1, \ldots, y_n$ are realizations of independent Gaussian random variables $Y_1, \ldots, Y_n$, each with $\mathsf{E}\, Y_i = \left\langle x_i, \beta^* \right\rangle$ and unit variance. In this setting, the $\ell_1$-regularized maximum-likelihood estimator is a natural choice:
\begin{equation}
\hat{\beta}_n := \arg \min_{\beta \in \mathbb{R}^p} \frac{1}{n} \sum_{i = 1}^n \ell ( y_i; \beta, x_i ) + \tau_n \left\Vert \beta \right\Vert_1, \notag
\end{equation}
where $\ell: \beta \mapsto ( 1/2 ) ( y_i - \left\langle x_i, \beta \right\rangle )^2$ denotes the negative log-likelihood at $y_i$ given $x_i$ and $\beta$. We obtain (\ref{eq_betahat}) with $L_n( \beta ) := \frac{1}{n} \sum_{i = 1}^n \ell( y_i; \beta, x_i )$, which is the well-known Lasso. The formulation \eqref{eq_betahat} readily extends to nonlinear models, such as sparse graphical learning~\cite{Ravikumar2011}. We will discuss the sparse graphical learning problem and some other applications in details in Section \ref{sec_appl}.

In this work, we specifically focus on the \emph{sparsistency} of $\hat{\beta}_n$, which is defined as follows
\begin{defn}[Sparsistency] \label{def_sparsistency}
An estimator $\hat{\beta}_n$ is called \emph{sparsistent} if there exists a sequence $\{ \tau_n \}_{n \in \mathbb{N}}$ such that
\begin{equation}
\lim_{n \to \infty} \mathsf{P}\, \left\{ \mathrm{supp}\, \hat{\beta}_n \neq \mathrm{supp}\, \beta^* \right\} = 0. \notag
\end{equation}
\end{defn}
Roughly speaking, an estimator $\hat{\beta}_n$ is sparsistent if it recovers the support of $\beta^*$ with overwhelming probability, when the number of samples $n$ is large enough. 

The main result of this paper is a sparsistency analysis framework that covers a wide variety of $\ell_1$-regularized $M$-estimators \eqref{eq_betahat}. We introduce a local condition, called as the local Kantorovich condition (LKC), and show how to obtain scaling laws of $( s, p )$ as a function of $n$ based on the LKC. To the best of our knowledge, we obtain the tightest sparsistency results for Gamma, logistics, and 

With the LKC 
 
%, if the function $L$ is convex and self-concordant, and certain irrepresentability-like condition \cite{Wainwright2009} holds true, then the $\ell_1$-regularized maximum-likelihood estimator $\hat{\beta}$ in (\ref{eq_betahat}) is sparsistent. This results is true even under the diverging dimensions case, where $p$ grows logarithmically with $n$, provided that $s := \left\Vert \beta^* \right\Vert_0 = o(n)$.

\paragraph{Our contributions in the context of prior work:} We have a good understanding of sparsistency guarantees (i.e., the number of samples required, the conditions imposed on the models, and so on) only for \emph{some special instances} of statistical models and $M$-estimators. A structured understanding of sparsistency for $\ell_1$-regularized $M$-estimators in general (and even for particular statistical model \emph{families}, such as generalized linear models, and exponential models) is still lacking.  

For the specific case of sparse linear regression, the class of $\ell_1$-regularized least squares estimators has received considerable attention. With respect to sparsistency, the results have ranged from exact recovery for noiseless observations (e.g.,~\cite{DonTan05,Donoho06,CandesTao05}), to sparsistency even with the noise~\cite{Meinshausen06,Wainwright2009,Zhao06}. 

The theory revolving around sparsistency however becomes involved when we move from linear regression models to the non-linear models. While  \mbox{$\ell_1$-regularized} estimators for the 
logistic and Gaussian Markov random field models have been shown to be sparsistent \cite{Ravikumar2010,Bunea08,Ravikumar2011,LamFan07,Meinshausen06}, the analysis for the general generalized linear model (GLM) case is still outstanding. 

%
%based on maximum likelihood have been shown to be sparsistent~, is still outstanding. Similarly, for the problem of estimating Gaussian Markov random fields, while the $\ell_1$-regularized MLE estimators have been shown to be model selection consistent, the analysis for the general

A key roadblock to such a general analysis has been the lack of identification of a general property of statistical models, and their corresponding $M$-estimators, that would enable the sparsistency analysis.\vcmargin{2bwritten}

%There has been considerable recent researches on high-dimensional estimation, including work on varied classes of estimators as well as their corresponding statistical analyses. In this paper, we are interested specifically in the class of $\ell_1$-regularized $M$-estimators for sparse high-dimensional estimation. A key motivation for adopting $\ell_1$-regularized $M$-estimators is model selection, or selecting the important entries of a high-dimensional parameter based on random observations; we are thus specifically interested in the sparsistency, that is the consistency in recovering the sparsity pattern or model selection consistency, of this class of estimators. For the specific case of sparse linear regression, the class of $\ell_1$-regularized least squares estimators (also called the Lasso~[REF]) has received considerable attention. With respect to sparsistency, the results have ranged from exact recovery for noiseless observations (e.g.,~\cite{DonTan05,Donoho06,CandesTao05}), to sparsistency even in the noisy setting~\cite{Meinshausen06,Wainwright2009,Zhao06}. These analyses however get trickier when moving from linear regression models to the non-linear setting. For the case of logistic regression  models, estimators based on \mbox{$\ell_1$-regularized} maximumlikelihood have again been shown to be model selection consistent~\cite{Ravikumar2010,Bunea08}; though an analysis for the general generalized linear model (GLM) case still seems outstanding. Similarly, for the problem of estimating Gaussian Markov random fields, the $\ell_1$-regularized MLE estimators have been shown to be model selection consistent~\cite{Ravikumar2011,LamFan07,Meinshausen06}, even while the analysis for the general exponential family distribution case seems outstanding.

%%%%%%%%%This work is interested in a \emph{class} of $\ell_1$-regularized $M$-estimators for sparse model selection. We focus on a key property of the estimators in this setting, called the sparsistency, which measures their success of recovering the unknown model's sparsity pattern. 
%%%%%%%%%
%%%%%%%%%For the specific case of sparse linear regression, the class of $\ell_1$-regularized least squares estimators has received considerable attention. With respect to sparsistency, the results have ranged from exact recovery for noiseless observations (e.g.,~\cite{DonTan05,Donoho06,CandesTao05}), to sparsistency even in the noisy setting~\cite{Meinshausen06,Wainwright2009,Zhao06}. The theory revolving around this topic however gets move involved when we move from linear regression models to the non-linear loss setting. While  \mbox{$\ell_1$-regularized} estimators for logistic regression based on maximum likelihood have been shown to be model selection consistent~\cite{Ravikumar2010,Bunea08}; though an analysis for the general generalized linear model (GLM) case still seems outstanding. Similarly, for the problem of estimating Gaussian Markov random fields, the $\ell_1$-regularized MLE estimators have been shown to be model selection consistent~\cite{Ravikumar2011,LamFan07,Meinshausen06}, even while the analysis for the general exponential family distribution case seems outstanding.
%%%%%%%%%
%%%%%%%%%
%%%%%%%%%
%%%%%%%%%We thus have a good understanding of sparsistency guarantees (the number of samples required, the conditions imposed on the models, and so on) only for \emph{some special instances} of statistical models and $M$-estimators; a structured understanding of sparsistency for $\ell_1$-regularized $M$-estimators in general (and even for particular statistical model \emph{families}, such as generalized linear models, and exponential models) is still lacking. A key roadblock to such a general analysis has been the lack of identification of a general property of statistical models, and their corresponding $M$-estimators, that would enable the sparsistency analyses.
%%%%%%%%%
%%%%%%%%%One could however specify some stringent conditions under which the sparsistency analyses would hold. Consider the following two smoothness conditions on the smooth component $L_n$ (that is, minus the $\ell_1$ regularization) of the $\ell_1$-regularized $M$-estimators:
%%%%%%%%%\begin{enumerate}
%%%%%%%%%\item \emph{Lipschitz-continuous gradient}: $\left\Vert \nabla L_n( y ) - \nabla L_n( x )  \right\Vert \leq L_g \left\Vert y - x \right\Vert$ with some $L_g \geq 0$, and
%%%%%%%%%\item \emph{Lipschitz-continuous Hessian}: $\left\Vert \nabla^2 L_n( y ) - \nabla^2 L_n( x )  \right\Vert \leq L_H \left\Vert y - x \right\Vert$ with some $L_H \geq 0$,
%%%%%%%%%\end{enumerate}
%%%%%%%%%and the strong convexity condition, $\left\langle \nabla L_n( y ) - \nabla L_n( x ), y - x \right\rangle \geq \mu \left\Vert y - x \right\Vert^2$ with some $\mu > 0$. We show in Section \ref{sec_summary_proof} that, with these common assumptions in optimization theory \cite{Nesterov2004}, it is direct to prove the sparsistency for $L_n$ that possess Lipschitz-continuous gradients/Hessians and are strongly convex. There are, however, some important applications with $L_n$ that don't satisfy those conditions. Examples include gamma and Poisson regression problems where the log-likelihood function involves the logarithmic function, and the graphical learning problem where the loss function involves the log-determinant function.
%%%%%%%%%
%%%%%%%%%In this paper, we introduce the property of locally uniform self-concordance, which is a property that is slightly stronger than that of vanilla self-concordance. As we argue in Section~\ref{Sec:LLH-LUSC}, vanilla self-concordance entails that the Hessian be locally Liptshitz in a very stringent ball around the current point, specifically, the radius of the ball is below the statistical precision, which renders it useless for statistical analyses. Our locally uniform self-concordance property on the other hand entails the Hessian satisfy a much less stringent locally Lipshitz property. As we show this suffices for us to provide a general sparsistency analysis for general $\ell_1$-regularized $M$-estimators. As we show in our corollaries, typical statistical model classes have MLEs that do indeed satisfy our local self-concordance property, which allows us to provide sparsistency guarantees for the corresponding $\ell_1$-regularized MLEs by a simple application of our main theorem.
%%%%%%%%%
%%%%%%%%%

\subsection*{Notations}

==> sections/lusc.tex <==
We define the class of locally smooth functions, and develop some basic properties.

\begin{defn}[Locally Smooth Functions] \label{def_SC}
Let $f \in C^3 ( \mathrm{dom}\, f )$ with open domain $\mathrm{dom}\, f \in \mathbb{R}^p$. The function is \emph{$( x, \mathcal{N}_x )$-locally smooth with parameter $L \geq 0$}  if
\begin{equation}
\left\vert D^3 f ( x + \delta ) [ u, u, u ] \right\vert \leq L \left\Vert u \right\Vert_2^3, \notag
\end{equation}
for the given point $x \in \mathrm{dom}\, f$, all $x + \delta \in \mathcal{N}_x \subseteq \mathrm{dom}\, f$, and all $u \in \mathbb{R}^p$.
\end{defn}

\begin{rem}
This is equivalent to saying that the Hessian is locally Lipschitz continuous.
\end{rem}

(Perhaps we should also show the following and its corresponding properties. I guess then the local smooth gradient condition alone does not suffice; we should also introduce the margin condition.)

\begin{defn}[Locally Uniformly Smooth Gradient] \label{def_SC}
Let $f \in C^2 ( \mathrm{dom}\, f )$ with open domain $\mathrm{dom}\, f \in \mathbb{R}^p$. The function has a \emph{$( x, \mathcal{N}_x )$-locally smooth gradient with parameter $L \geq 0$}  if
\begin{equation}
\left\vert D^2 f ( x + \delta ) [ u, u ] \right\vert \leq L \left\Vert u \right\Vert_2^2, \notag
\end{equation}
for the given point $x \in \mathrm{dom}\, f$, all $x + \delta \in \mathcal{N}_x \subseteq \mathrm{dom}\, f$, and all $u \in \mathbb{R}^p$.
\end{defn}

Since $D^3 f (x)$ and $\left\Vert \cdot \right\Vert_2^2$ are symmetric linear forms, we have the following theorem based on~\cite[Appendix 1]{Nesterov1994}.

\begin{thm} \label{thm_equiv_def_sc}
Let $f \in C^3( \mathrm{dom}\, f )$ with open domain $\mathrm{dom}\, f \subset \mathbb{R}^p$. The function $f$ is $( x, \mathcal{N}_x )$-locally smooth with parameter $L \geq 0$ if and only if
\begin{equation}
\left\vert D^3 f( x + \delta ) [ u_1, u_2, u_3 ] \right\vert \leq L \prod_{i = 1}^3 \left\Vert u_i \right\Vert_2 \notag
\end{equation}
for the given point $x \in \mathrm{dom}\, f$, all $x + \delta \in \mathcal{N}_x \subseteq \mathrm{dom}\, f$, and all $u_1, u_2, u_3 \in \mathbb{R}^p$.
\end{thm}

The local smoothness property is preserved under linear combinations with positive coefficients.

\begin{lem} \label{lem_preservation_sc} 
Let $f_1$ be $( x, \mathcal{N}_{1} )$-locally smooth with parameter $M_1$, and $f_2$ be $( x, \mathcal{N}_{2} )$-locally smooth with parameter $M_2$. Let $\alpha$ and $\beta$ be two positive real numbers. The function $f := \alpha f_1 + \beta f_2$ is $( x, \mathcal{N}_x )$-locally smooth with parameter $M$, where $\mathcal{N}_x := \mathcal{N}_1 \cap \mathcal{N}_2$, and $M := \alpha M_1 + \beta M_2$.
\end{lem}

We note that this is related to, and \emph{weaker} than the self-concordance property \cite{Nesterov1994,Nesterov2004}, which would entail that:
\[D^3 f ( x + \delta)[u,u,u] \le L \| u \|_{ x + \delta}^3,\]
where $\| u\|_x = (D^2 f( x )[u,u])^{1/2}$.
Noting that
\[ \| u\|_{x + \delta} = (D^2 f ( x + \delta)[u,u])^{1/2} \le \kappa_{\max} \| u\|^2,\]
where $\kappa_{\max} = \lambda_{\max}(D^2 f ( x + \delta))$, it follows that when the loss is self-concordant with parameter
$\kappa$, it will satisfy the local-Lipshitz property with parameter $\kappa \,\kappa_{\max}^{3}$. 

The converse however would require a bound of the form $\| u \|_{x + \delta} \le \kappa' \|u\|$, which would require that the Hessian be invertible, so that $\lambda_{\min}(D^2 f ( x + \delta)) > 0$, which might not hold in high-dimensional settings. Indeed, the high-dimensional settings seem ill-suited to the self-concordance property: the upper bound required in the self-concordance property might not hold for $u$ in the null-space of $D^2f ( x + \delta)$: when the Hessian is not full rank, $\| u\|_x = (D^2 f ( x )[u,u])^{1/2} = 0$.

%In order to prove the sparsistency result, we relax the definition of self-concordant functions in the following manner.
%
%\begin{defn}[Locally Uniformly Self-Concordant (LUSC) Functions] \label{def_lusc}
%Let $f \in C^3 ( \mathrm{dom}\, f )$ be a closed convex function with open domain $\mathrm{dom}\, f \subset \mathbb{R}^p$. Let $x \in \mathrm{dom}\, f$ and $\mathcal{N}_x$ be a subset of $\mathrm{dom}\, f$ containing $x$. The function $f$ is \emph{$( x, \mathcal{N}_x )$-locally uniformly self-concordant ($( x, \mathcal{N}_x )$-LUSC) with parameter $M \geq 0$} if and only if
%\begin{equation}
%\left\vert D^3 f( x + \delta ) [ u, u, u ] \right\vert \leq M \left( D^2 f( x ) [ u, u ] \right)^{3/2} \notag
%\end{equation}
%for the given point $x \in \mathrm{dom}\, f$, all $\delta$ such that $x + \delta \in \mathcal{N}_x$, and all $u \in \mathbb{R}^p$.
%\end{defn}
%
%This definition relaxes the original definition in the following two aspects. First, we only consider the local behavior of $f$ on a neighborhood of the point $x$. Second, we allow the input of the mapping $D^3 f ( \cdot )$ to be perturbed by a vector $\delta$. The first is weaker than the self-concordance property while the second is locally stronger.
%
%Following the derivations in \cite{Nesterov1994,Nesterov2004}, we have the following results analogous to Theorem \ref{thm_equiv_def_sc} and Lemma \ref{lem_preservation_sc} respectively.
%
%\begin{thm} \label{thm_equiv_def_lusc}
%Let $f \in C^3 ( \mathrm{dom}\, f )$ be a closed convex function with open domain $\mathrm{dom}\, f \subset \mathbb{R}^p$. Let $x \in \mathrm{dom}\, f$ and $\mathcal{N}_x$ be a subset of $\mathrm{dom}\, f$ containing $x$. The function $f$ is $( x, \mathcal{N}_x )$-LUSC with parameter $M \geq 0$ if and only if
%\begin{equation}
%\left\vert D^3 f( x + \delta ) [ u_1, u_2, u_3 ] \right\vert \leq M \prod_{i = 1}^3 \left( D^2 f( x )[ u_i, u_i ] \right)^{1/2} \notag
%\end{equation}
%for the given point $x \in \mathrm{dom}\, f$, all $\delta$ such that $x + \delta \in \mathcal{N}_x$, and all $u_1, u_2, u_3 \in \mathbb{R}^p$.
%\end{thm}
%
%\begin{lem} \label{lem_preservation_lusc}
%Let $f_1$ be $( x, \mathcal{N}_{1} )$-LUSC with parameter $M_1$, and $f_2$ be $( x, \mathcal{N}_{2} )$-LUSC with parameter $M_2$. Let $\alpha$ and $\beta$ be two positive real numbers. The function $f := \alpha f_1 + \beta f_2$ is $( x, \mathcal{N}_x )$-LUSC with parameter $M$, where $\mathcal{N}_x := \mathcal{N}_1 \cap \mathcal{N}_2$, and $M := \max \left\{ M_1 / \sqrt{\alpha}, M_2 / \sqrt{\beta} \right\}$.
%\end{lem}
%
%The proofs are similar to the corresponding proofs in \cite{Nesterov1994,Nesterov2004} for Theorem \ref{thm_equiv_def_sc} and Lemma \ref{lem_preservation_sc}, so we omit them.

% The local strong convexity condition is crucial in bounding the estimation error of an $M$-estimator, as we shall see in Appendix \ref{}.
% 
% \begin{defn}[$( x, \mathcal{F}_x )$-Local Strong Convexity]
% A differentiable function $f: \mathrm{dom}\, f \to \mathbb{R}$ is called $( x, \mathcal{F}_x )$-locally strongly convex with parameter $\mu > 0$ if
% \begin{equation}
% f( y ) - f( x ) \geq \left\langle \nabla f( x ), y - x \right\rangle + \frac{\mu}{2} \left\Vert y - x \right\Vert^2, \notag
% \end{equation}
% for all $y \in \mathcal{F}_x \subseteq \mathrm{dom}\, f$, for the given $x \in \mathrm{dom}\, f$. 
% \end{defn}
% 
% \begin{rem}
% This condition is essentially an instance of the \emph{margin condition} in \cite{Buhlmann2011}; we choose this formulation simply for convenience. This local strong convexity condition is closely related to and in general weaker than the \emph{restricted strong convexity condition} \cite{Negahban2012}. When the Hessian is a constant, this reduces to the \emph{restricted eigenvalue condition} \cite{Bickel2009}.
% \end{rem}
% 
% \begin{rem}
% When $f \in C^2( \mathrm{dom}\, f )$, it is sufficient to require $\nabla^2 f( y ) \geq \mu I$ for all $y \in \mathcal{F}_x$, since
% \begin{equation}
% f( y ) - f( x ) = \left\langle \nabla f( x ), y - x \right\rangle + \frac{1}{2} \left\langle y - x, G ( y - x ) \right\rangle, \notag
% \end{equation}
% with 
% \begin{equation}
% G = \int_{0}^1 \nabla^2 f[ x + t ( y - x ) ] \, dt. \notag
% \end{equation}
% \end{rem}
% 
% \begin{rem}
% Usually it suffices to require that $\nabla^2 f(x) \geq \rho I$ with some $\rho > 0$, for the given $x$. When the Hessian is continuous, there exists some $\mathcal{F}_x$ such that $\nabla^2 f( y ) \geq \mu I$ with some $\rho \geq \mu > 0$ for all $y \in \mathcal{F}_x$.
% \end{rem}
% 
% By definition we have the following lemma.
% 
% \begin{lem} \label{lem_preservation_lsc}
% Let $f_1$ be $( x, \mathcal{F}_1 )$-locally strongly convex and $f_2$ be $( x, \mathcal{F}_2 )$-locally strongly convex, with parameters $\mu_1$ and $\mu_2$ respectively. Let $\alpha$ and $\beta$ be two positive numbers. Then the function $f := \alpha f_1 + \beta f_2$ is $( x, \mathcal{F} )$-locally strongly convex with parameter $\alpha \mu_1 + \beta \mu_2$, where $\mathcal{F} = \mathcal{F}_1 \cap \mathcal{F}_2$.
% \end{lem}

%\subsection{Locally Lipshitz Hessians and Local Self-Concordance}
%\label{Sec:LLH-LUSC}

% This condition is essentially an instance of the \emph{margin condition} in \cite{Buhlmann2011}; we choose this formulation simply for convenience. This local strong convexity condition is closely related to and in general weaker than the \emph{restricted strong convexity condition} \cite{Negahban2012}. When the Hessian is a constant, this reduces to the \emph{restricted eigenvalue condition} \cite{Bickel2009}.


==> sections/main_proof.tex <==
% For the locally Lipschitz continuous Hessian assumption

It is desirable to have $\hat{\beta}_n = \check{\beta}_n$ and $\mathrm{supp}\, \check{\beta}_n = \mathrm{supp}\, \beta^*$, since then the support consistency is established. We derive sufficient conditions for $\hat{\beta}_n = \check{\beta}_n$ in Lemma \ref{lem_PDW}, and make the sufficient condition explicit and upper-bound $\left\Vert \check{\beta} - \beta^* \right\Vert_2$ in Lemma \ref{lem_quasi_support_consistency}. Then sign consistency follows if $\beta_{\min}$ is strictly larger than the error bound.

The following lemma can be derived in a similar way as in \cite{Wainwright2009}. We skip the proof here.

\begin{lem} \label{lem_PDW}
We have $\hat{\beta}_n = \check{\beta}_n$ if
\begin{equation}
\left\Vert \left[ \nabla L_n( \check{\beta}_n ) \right]_{\mathcal{S}^{\mathrm{C}}} \right\Vert_{\infty} < \tau_n. \notag
\end{equation}
\end{lem}

\begin{rem}
Thus if the condition in Lemma \ref{lem_PDW} is satisfied, the estimator $\hat{\beta}_n$ exists and is unique as $\check{\beta}$.
\end{rem}

We now derive explicit conditions for $\hat{\beta}_n = \check{\beta}_n$.

\begin{lem} \label{lem_quasi_support_consistency}
With the assumptions in Section \ref{sec_assumptions}, we have $\hat{\beta}_n = \check{\beta}_n$ if
\begin{equation}
\left\Vert \left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}^{\mathrm{C}}, \mathcal{S}} \left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}}^{-1} \right\Vert_{\infty} < 1 - \alpha \notag
\end{equation}
with some $\alpha \in (0, 1]$, 
\begin{equation}
\left\Vert \nabla L_n( \beta^* ) \right\Vert_\infty \leq \frac{\alpha}{4} \tau_n, \notag
\end{equation}
and $\check{\beta} \in \mathcal{N}_{\beta^*} \cap \mathcal{B}_{\beta^*}$, where
\begin{equation}
\mathcal{B}_{\beta^*} := \left\{ \beta: \left\Vert \check{\beta}_n - \beta^* \right\Vert_{\beta^*} \leq \sqrt{\frac{\alpha \tau_n}{2 \sigma M_{n, \beta^*}}}, \beta_{\mathcal{S}^c} = 0, \beta \in \mathbb{R}^p \right\}. \notag
\end{equation}
\end{lem}

\begin{proof}
By Taylor expansion at $\beta^*$, we obtain
\begin{equation}
\left[ \nabla L( \check{\beta}_n ) \right]_{\mathcal{S}^{\mathrm{C}}} = \left[ \nabla L_n( \beta^* ) \right]_{\mathcal{S}^{\mathrm{C}}} + \left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}^{\mathrm{C}}, \mathcal{S}} \left( \check{\beta}_n - \beta^* \right)_{\mathcal{S}} + \left( r_n \right)_{\mathcal{S}^{\mathrm{C}}}, \label{eq_taylor_1}
\end{equation}
where $r_n$ is the remainder term whose $k$-th element is 
\begin{equation}
\left( r_n \right)_k := \frac{1}{2} D^3 L_n( \tilde{\beta}_k ) [ e_k, \check{\beta}_n - \beta^*, \check{\beta}_n - \beta^* ] \notag
\end{equation}
with some $\tilde{\beta}_k \in [ \beta^0, \check{\beta} ]$ for $k \in \{ 1, \ldots, p \}$. We define the vector $e_k$ as $e_k := ( \delta_{i,k} )_{i \in \{ 1, \ldots, p \}}$, where $\delta$ denotes the Kronecker delta.

The optimality condition for $\check{\beta}_n$ is
\begin{equation}
\left[ \nabla L_n( \check{\beta}_n ) \right]_{\mathcal{S}} + \tau_n \check{z}_{\mathcal{S}} = 0, \notag
\end{equation}
with some $\check{z} \in \partial \left\Vert \check{\beta}_n \right\Vert_1$. By the Taylor expansion again, we have
\begin{equation}
\left[ \nabla L_n( \check{\beta}_n ) \right]_{\mathcal{S}} + \left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}} \left( \check{\beta}_n - \beta^* \right)_{\mathcal{S}} + (r_n)_{\mathcal{S}} + \tau_n \check{z}_{\mathcal{S}} = 0. \label{eq_taylor_2}
\end{equation}

Solve $\left( \check{\beta}_n - \beta^* \right)_{\mathcal{S}}$ in (\ref{eq_taylor_2}) and substitute the solution in (\ref{eq_taylor_1}). We obtain
\begin{align}
\left[ \nabla L_n( \check{\beta}_n ) \right]_{\mathcal{S}^{\mathrm{C}}} &= - \tau_n \left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}^{\mathrm{C}}, \mathcal{S}} \left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}}^{-1} \check{z}_{\mathcal{S}} \notag \\
&\quad\,\, + \left[ \nabla L( \beta^* ) \right]_{\mathcal{S}^{\mathrm{C}}} - \left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}^{\mathrm{C}}, \mathcal{S}} \left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}}^{-1} \left[ \nabla L_n( \beta^* ) \right]_{\mathcal{S}} \notag \\
&\quad\,\, + ( r_n )_{\mathcal{S}^{\mathrm{C}}} - \left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}^{\mathrm{C}}, \mathcal{S}} \left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}}^{-1} ( r_n )_{\mathcal{S}}. \notag
\end{align}
By the triangle inequality, we have $\left\Vert \left[ \nabla L_n( \check{\beta}_n ) \right]_{\mathcal{S}^{\mathrm{C}}} \right\Vert_{\infty} < \tau_n$ if the irrepresentability condition (\ref{eq_irrepresentability}) holds, and
\begin{equation}
\max \left\{ \left\Vert \nabla L_n( \beta^* ) \right\Vert_{\infty}, \left\Vert r_n \right\Vert_{\infty} \right\} \leq \frac{\alpha}{4} \tau_n. \notag
\end{equation}
The first requirement that $\left\Vert \nabla L_n( \beta^* ) \right\Vert_{\infty} \leq ( \alpha / 4 ) \tau_n$ is satisfied by assumption. 

We now derive sufficient conditions for $\left\Vert r_n \right\Vert_{\infty} \leq ( \alpha / 4 ) \tau_n$. Since $L_n$ is $( \beta^*, \mathcal{N}_{\beta^*} )$-LUSC with parameter $\sqrt{n}$, we have, by Theorem \ref{thm_equiv_def_lusc}, 
\begin{align}
\left\vert ( r_n )_k \right\vert \leq \frac{M_{n, \beta^*}}{2} \left\Vert e_k \right\Vert_{\beta^*} \left\Vert \check{\beta}_n - \beta^* \right\Vert_{\beta^*}^2 \leq \frac{M_{n, \beta^*} \sigma}{2} \left\Vert \check{\beta}_n - \beta^* \right\Vert_{\beta^*}^2. \notag
\end{align}
for all $k \in \{ 1, \ldots, p \}$, given that $\check{\beta}_n \in \mathcal{N}_{\beta^*}$. 
Thus, in order to have $\left\Vert r_n \right\Vert_\infty \leq ( \alpha / 4 ) \tau_n$, it suffices to require
\begin{equation}
\left\Vert \check{\beta}_n - \beta^* \right\Vert_{\beta^*} \leq \sqrt{\frac{\alpha \tau_n}{2 \sigma M_{n, \beta^*}}}. \notag
\end{equation}

\end{proof}

To bound the distance $\left\Vert \check{\beta} - \beta^* \right\Vert_{\beta^*}$, we adopt the following approach from \cite{Rothman2008,Ravikumar2010}. We make the statements rigorous below.

\begin{lem}
Let $g: \mathbb{R}^p \to \mathbb{R}$ be a convex function, and let $x \in \mathbb{R}^p$ such that $g( x ) \leq 0$. Let $\mathcal{B} \subset \mathbb{R}^p$ be a closed set and $\partial \mathcal{B}$ be its boundary. If $g > 0$ on $\partial \mathcal{B}$ and $g( o ) \leq 0$ for some $o \in \mathcal{B} \setminus \partial \mathcal{B}$, then $x \in \mathcal{B}$.
\end{lem}
\begin{proof}
We prove by contradiction. Suppose that $x \notin \mathcal{B}$. We claim there exists some $t^* \in ( 0, 1 )$ such that $o + t^* ( x - o ) \in \partial \mathcal{B}$, since if such $t^*$ does not exist, then $x_{t_n} := o + t_n^* ( x - o ) \to x \in \mathcal{B}$ as $t_n \to 1$, a contradiction.

By the convexity of $g$, we have
\begin{equation}
g( o + t^* ( x - o ) ) \leq ( 1 - t^* ) g( o ) + t g( x ) \leq 0, \notag
\end{equation}
a contradiction.
\end{proof}

Now we prove that $\left\Vert \check{\beta} - \beta \right\Vert_{\beta^*}$ is bounded.

\begin{lem}
With the assumptions in Section \ref{sec_assumptions}, we have 
\begin{equation}
\check{\beta}_n \in \mathcal{B}_{R_n} := \left\{ \left\Vert \check{\beta}_\mathcal{S} - \beta^*_{\mathcal{S}} \right\Vert_2 \leq R_n \right\}, \notag \end{equation}
where $R_n$ is some constant satisfying
\begin{equation}
R_n > \left( 1 + \frac{\alpha}{4} \right) \frac{2 \tau_n}{\mu} \sqrt{s}, \notag
\end{equation}
given that $\mathcal{B}_{R_n} \subseteq \mathcal{F}_{\beta^*}$.
\end{lem}

\begin{proof}
Let $s = \left\vert \mathcal{S} \right\vert$. Let $Z: \beta \in \mathbb{R}^s \mapsto ( \beta, 0 ) \in \mathbb{R}^p$ be the zero-padding mapping, where $( \beta, 0 )$ denotes the vector $v$ that equals to $\beta$ on $\mathcal{S}$ and $0$ on $\mathcal{S}^{\mathrm{c}}$. Then we have
\begin{equation}
\check{\beta}_{\mathcal{S}} = \arg \min_{\beta \in \mathbb{R}^s} \left\{ ( L \circ Z )( \beta ) + \tau_n \left\Vert \beta \right\Vert_1 \right\}. \notag
\end{equation}
Define 
\begin{equation}
g: \delta \in \mathbb{R}^s \mapsto ( L_n \circ Z )( \beta_{\mathcal{S}}^* + \delta ) - ( L_n \circ Z )( \beta_{\mathcal{S}}^* ) + \tau_n \left( \left\Vert \beta_{\mathcal{S}}^* + \delta \right\Vert_1 - \left\Vert \beta_{\mathcal{S}}^* \right\Vert_1 \right), \notag
\end{equation}
where $( \delta, 0 )$ denotes the vector $v \in \mathbb{R}^p$ that equals to $\delta$ on $\mathcal{S}$ and $0$ on $\mathcal{S}^{\mathrm{c}}$. By definition $g(0) = 0$, and thus $g( \delta^* ) \leq 0$. Now our goal is to find some constant $r > 0$ such that $g > 0$ on $\partial \mathcal{B}_{R_n}$, where $\mathcal{B} := \left\{ \delta \in \mathbb{R}^s : \left\Vert \delta \right\Vert_2\leq r \right\}$. Then by the previous lemma, $\delta^* \in \mathcal{B}$, i.e., $\left\Vert \check{\beta} - \beta^* \right\Vert_{\beta^*} \leq r$.

Now we derive a lower bound on $g( \delta )$. We have, since $( L_n \circ Z )$ is $( \beta^*, \mathcal{F}_{\beta^*} )$-locally strongly convex with parameter $\mu$,
\begin{align}
( L_n \circ Z )( \beta^* + ( \delta, 0 ) ) - ( L_n \circ Z )( \beta^* ) \geq \left\langle \left[ \nabla L_n( \beta^* ) \right]_{\mathcal{S}}, \delta \right\rangle  + \frac{\mu}{2} \left\Vert \delta \right\Vert_2^2, \notag
\end{align}
given that $\beta^* + ( \delta, 0 ) \in \mathcal{F}_{\beta^*}$. By H\"{o}lder's inequality, 
\begin{equation}
\left\vert \left\langle \left[ \nabla L_n( \beta^* ) \right]_{\mathcal{S}}, \delta \right\rangle \right\vert \leq \left\Vert \left[ \nabla L_n( \beta^* ) \right]_{\mathcal{S}} \right\Vert_{\infty} \left\Vert \delta \right\Vert_1 \leq \frac{\alpha \tau_n}{4} \left\Vert \delta \right\Vert_1 \leq \frac{\alpha \tau_n \sqrt{s}}{4} \left\Vert \delta \right\Vert_2. \notag
\end{equation}
By the triangle inequality, 
\begin{equation}
\left\vert \tau_n \left( \left\Vert \beta_{\mathcal{S}}^* + \delta \right\Vert_1 - \left\Vert \beta_{\mathcal{S}}^* \right\Vert_1 \right) \right\vert \leq \tau_n \left\Vert \delta \right\Vert_1 \leq \tau_n \sqrt{s} \left\Vert \delta \right\Vert_2. \notag
\end{equation}
Thus we obtain
\begin{equation}
g( \delta ) \geq - \frac{\alpha \tau_n \sqrt{s}}{4} \left\Vert \delta \right\Vert_2 + \frac{\mu}{2} \left\Vert \delta \right\Vert_2^2 - \tau_n \sqrt{s} \left\Vert \delta \right\Vert_2. \notag
\end{equation}
Thus, by choosing
\begin{equation}
R_n > \left( 1 + \frac{\alpha}{4} \right) \frac{2 \tau_n}{\mu} \sqrt{s}, \notag
\end{equation}
we have $g > 0$ on $\partial \mathcal{B}_{R_n}$.
\end{proof}

% Previous versions without the local strong convexity assumption

\begin{lem}
With the assumptions in Section \ref{sec_assumptions}, we have 
\begin{equation}
\check{\beta}_n \in \mathcal{B}_{R_n} := \left\{ \left\Vert \check{\beta}_\mathcal{S} - \beta^*_{\mathcal{S}} \right\Vert_{\left[ \nabla^2 L_n ( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}}} \leq R_n \right\}, \notag \end{equation}
where $R_n$ is some positive number satisfying
\begin{equation}
R_n > \frac{3}{2 M_{n, \beta^*}} + \sqrt{ \frac{6}{M_{n, \beta^*}} \left( \frac{3}{8 M_{n, \beta^*}} - 2 \sqrt{\frac{s}{\lambda_{\min}}} \tau_n \right) }, \notag
\end{equation}
given that $\mathcal{B}_{R_n} \subseteq \mathcal{N}_{\beta^*}$, and 
\begin{equation}
\tau_n \leq \frac{3}{16 M_{n, \beta^*}} \sqrt{\frac{\lambda_{\min}}{s}}. \notag
\end{equation}
\end{lem}

\begin{proof}
Let $s = \left\vert \mathcal{S} \right\vert$. Let $Z: \beta \in \mathbb{R}^s \mapsto ( \beta, 0 ) \in \mathbb{R}^p$ be the zero-padding mapping, where $( \beta, 0 )$ denotes the vector $v$ that equals to $\beta$ on $\mathcal{S}$ and $0$ on $\mathcal{S}^{\mathrm{c}}$. Then we have
\begin{equation}
\check{\beta}_{\mathcal{S}} = \arg \min_{\beta \in \mathbb{R}^s} \left\{ ( L \circ Z )( \beta ) + \tau_n \left\Vert \beta \right\Vert_1 \right\}. \notag
\end{equation}
Define 
\begin{equation}
g: \delta \in \mathbb{R}^s \mapsto ( L_n \circ Z )( \beta_{\mathcal{S}}^* + \delta ) - ( L_n \circ Z )( \beta_{\mathcal{S}}^* ) + \tau_n \left( \left\Vert \beta_{\mathcal{S}}^* \right\Vert_1 - \left\Vert \beta_{\mathcal{S}}^* \right\Vert_1 \right), \notag
\end{equation}
where $( \delta, 0 )$ denotes the vector $v \in \mathbb{R}^p$ that equals to $\delta$ on $\mathcal{S}$ and $0$ on $\mathcal{S}^{\mathrm{c}}$. By definition $g(0) = 0$, and thus $g( \delta^* ) \leq 0$. Now our goal is to find some constant $r > 0$ such that $g > 0$ on $\partial \mathcal{B}$, where $\mathcal{B} := \left\{ \delta \in \mathbb{R}^s : \left\Vert \delta \right\Vert_{\left[ \nabla^2 L_n( \beta ) \right]_{\mathcal{S}, \mathcal{S}}} \leq r \right\}$. Then by the previous lemma, $\delta^* \in \mathcal{B}$, i.e., $\left\Vert \check{\beta} - \beta^* \right\Vert_{\beta^*} \leq r$.

Now we derive a lower bound on $g( \delta )$. Define $\phi(t) = ( L_n \circ Z )( \beta_\mathcal{S}^* + t \delta )$. Then we have
\begin{align}
( L_n \circ Z )( \beta^* + ( \delta, 0 ) ) - ( L_n \circ Z )( \beta^* ) = \phi(1) - \phi(0) = \phi'(0) + \frac{1}{2} \phi''(0) + \frac{1}{6} \phi'''( \tilde{t} ), \notag
\end{align}
with some $\tilde{t} \in [ 0, 1 ]$. For the term $\phi'(0)$, we have by H\"{o}lder's inequality,
\begin{align}
\left\vert \phi'(0) \right\vert &= \left\vert \left\langle \left[ \nabla L_n( \beta^* ) \right]_{\mathcal{S}},\delta  \right\rangle \right\vert \notag \\
&\leq \sqrt{ \frac{s}{\lambda_{\min}} } \left\Vert \left[ \nabla L_n( \beta^* ) \right]_{\mathcal{S}} \right\Vert_\infty \left\Vert \delta \right\Vert_{\left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}}} \leq \sqrt{\frac{s}{\lambda_{\min}}} \tau_n \left\Vert \delta \right\Vert_{\left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}}}. \notag
\end{align}
For the term $\phi''(0)$, we have 
\begin{equation}
\phi '' ( 0 ) = \left\Vert \delta \right\Vert_{\left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}}}^2. \notag
\end{equation}
For the term $\phi'''( \tilde{t} )$, we have
\begin{equation}
\left\vert \phi'''( \tilde{t} ) \right\vert = \left\vert D^3( L \circ Z ) ( \beta_{\mathcal{S}}^* + \tilde{t} \delta ) [ \delta, \delta, \delta ] \right\vert \leq M \left\Vert \delta \right\Vert_{ \left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}} }^3\notag
\end{equation}
given $\check{\beta} \in \mathcal{N}_{\beta^*}$. Finally, by the triangle inequality, we obtain
\begin{equation}
\left\vert \left\Vert \beta^* + ( \delta, 0 ) \right\Vert_1 - \left\Vert \beta^* \right\Vert_1 \right\vert \leq \left\Vert \delta \right\Vert_1 \leq \sqrt{\frac{s}{\lambda_{\min}}} \left\Vert \delta \right\Vert_{\left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}}} \notag
\end{equation}
given $\check{\beta} \in \mathcal{N}_{\beta^*}$. Therefore, $g( \delta ) \geq f \left( \left\Vert \delta \right\Vert_{\left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}}} \right)$ given $\check{\beta} \in \mathcal{N}_{\beta^*}$, where
\begin{equation}
f: x \mapsto - \sqrt{\frac{s}{\lambda_{\min}}} \tau_n x + \frac{1}{2} x^2 - \frac{M}{6} x^3 - \sqrt{\frac{s}{\lambda_{\min}}} \tau_n x = - 2 \sqrt{\frac{s}{\lambda_{\min}}} \tau_n x + \frac{1}{2} x^2 - \frac{M}{6} x^3. \notag
\end{equation}
The lemma follows by solving the inequality
\begin{equation}
f \left( \left\Vert \delta \right\Vert_{\left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}}} \right) > 0. \notag
\end{equation}
Note that we have to require $\mathcal{B}_{R_n} \subseteq \mathcal{N}_{\beta^*}$ to ensure that the bound on $\phi'''( \tilde{t} )$ is valid.
\end{proof}

%\begin{lem}
%With the assumptions in Section \ref{sec_assumptions}, we have
%\begin{equation}
%\left\Vert \check{\beta} - \beta^* \right\Vert_{\beta^*} \leq \frac{2}{M_n} \left[ \frac{W_{-1} \left(- \gamma e^{-\gamma} \right) }{- \gamma} - 1 \right], \notag
%\end{equation}
%where $W_{-1}$ denotes the Lambert $W$ function of the non-principal branch, implicitly defined as the solution of $W_{-1}(x) e^{W_{-1}(x)} = x$ satisfying $W_{-1}(x) \leq -1$, and
%\begin{equation}
%\gamma := 1 - \frac{M_n}{2} \left( 1 + \frac{\alpha}{4} \right) \tau_n \sqrt{\frac{s}{\lambda_{\min}}}, \notag
%\end{equation}
%given that
%\begin{equation}
%\tau_n \leq \frac{8}{\left( 4 + \alpha \right) M_n} \sqrt{\frac{\lambda_{\min}}{s}}. \notag
%\end{equation}
%\end{lem}
%\begin{proof}
%Let $Z: \beta \in \mathbb{R}^s \mapsto ( \beta, 0 ) \in \mathbb{R}^p$ be the zero-padding mapping, where $( \beta, 0 )$ denotes the vector $v$ that equals to $\beta$ on $\mathcal{S}$ and $0$ on $\mathcal{S}^{\mathrm{c}}$. Then we have
%\begin{equation}
%\check{\beta}_{\mathcal{S}} = \arg \min_{\beta \in \mathbb{R}^s} \left\{ ( L \circ Z )( \beta ) + \tau_n \left\Vert \beta \right\Vert_1 \right\}. \notag
%\end{equation}
%Thus
%\begin{equation}
%( L_n \circ Z )( \check{\beta}_\mathcal{S} ) - ( L_n \circ Z )( \beta^*_{\mathcal{S}} ) + \tau_n \left( \left\Vert \check{\beta}_{\mathcal{S}} \right\Vert_1 - \left\Vert \beta^*_{\mathcal{S}} \right\Vert_1 \right) \leq 0. \notag
%\end{equation}
%Let $\delta := \check{\beta}_{\mathcal{S}} - \beta^*_{\mathcal{S}}$. By the self-concordance of $L \circ Z$, we have
%\begin{equation}
%( L_n \circ Z )( \check{\beta}_\mathcal{S} ) - ( L_n \circ Z )( \beta^*_{\mathcal{S}} ) \geq \left\langle \left[ \nabla L_n( \beta^* ) \right]_{\mathcal{S}}, \delta \right\rangle + \omega \left( \left\Vert \delta \right\Vert_{\left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}}} \right), \notag
%\end{equation}
%where $\omega: x \mapsto 2 M_n^{-1} x - 4 M_n^{-2} \ln \left( 1 + 2^{-1} M_n x \right)$ \cite{Nesterov2004}, and thus, by the triangle inequality and H\"{o}lder's inequality,
%\begin{equation}
%- \left\Vert \left[ \nabla L_n ( \beta^* ) \right]_{\mathcal{S}} \right\Vert_{\infty} \left\Vert \delta \right\Vert_1  + \omega \left( \left\Vert \delta \right\Vert_{\left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}}} \right) \leq \tau_n \left\Vert \delta \right\Vert_1. \notag
%\end{equation} 
%With our assumption on the restricted Hessian, this implies
%\begin{equation}
%\ln \left( 1 + \frac{M_n}{2} \left\Vert \delta \right\Vert_{ \left[ \nabla^2 L_n ( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}} } \right) \geq \frac{M_n}{2} \left[ 1 - \frac{M_n}{2} \left( 1 + \frac{\alpha}{4} \right) \tau_n \sqrt{\frac{s}{\lambda_{\min}}} \right] \left\Vert \delta \right\Vert_{ \left[ \nabla^2 L_n ( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}} }, \notag
%\end{equation}
%where we use the fact that
%\begin{equation}
%\left\Vert \delta \right\Vert_1 \leq \sqrt{s} \left\Vert \delta \right\Vert_2 = \sqrt{s} \left\Vert \left[ \nabla^2 L_n ( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}}^{1/2} \delta \right\Vert_{ \left[ \nabla^2 L_n ( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}}^{-1} } \leq \sqrt{\frac{s}{\lambda_{\min}}} \left\Vert \delta \right\Vert_{ \left[ \nabla^2 L_n ( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}} }. \notag
%\end{equation}
%To ensure the existence of a positive solution for $\left\Vert \delta \right\Vert_{\left[ \nabla^2 L_n ( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}}}$, we require
%\begin{equation}
%\tau_n \leq \frac{8}{\left( 4 + \alpha \right) M_n} \sqrt{\frac{\lambda_{\min}}{s}}. \notag
%\end{equation}
%
%The lemma follows by the definition of Lambert $W$ function.
%\end{proof}


% \section{Proof of Corollary \ref{cor_main_deterministic}}

% Previous version without the local strong convexity

%Recall that $R_n$ is the positive solution of the equation 
%\begin{equation}
%\ln\left( 1 + \frac{M_n}{2} R_n \right) = \frac{M_n}{2}\left( 1 - \eta_n \right) R_n \label{eq_defRn}
%\end{equation}
%with some $\eta_n \in ( 0, 1 )$. Note that $R_n$ is uniquely defined.
%
%\begin{prop} \label{prop_ln1+x}
%Let $\gamma_n$ be a monotonically decreasing sequence converging to $0$. When $n$ is large enough such that $\gamma_n \leq 0.26$, we have $\sqrt{2} \gamma_n \leq R_n \leq \sqrt{3} \gamma_n$.
%\end{prop}
%
%\begin{proof}
%We first show that $\left\{ R_i \right\}_{i \in \mathbb{N}}$ as defined in (\ref{eq_defRn}) is also monotonically decreasing and converges to $0$. Define $f: x \mapsto x^{-1} \ln ( 1 + x )$. Then we have $f( R_n ) = ( 1 - \gamma_n )$. The sequence $\{ R_i \}_{i \in \mathbb{N}}$ is monotonically decreasing because $f$ is strictly decreasing, and $R_n \to 0$ as $n \to \infty$ because $f(x) \to 1$ as $x \to 0$.
%
%Let $N$ be the smallest integer such that $\gamma_n \leq 0.26$. Then, when $n \geq N$, we have $R_n \leq 0.78$. It can be checked that $u: x \mapsto x - \frac{1}{3} x^2$ is an upper bound of $h: x \mapsto \ln( 1 + x )$, and thus the solution of $u( x ) = ( 1 - \gamma_n ) x$ is an upper bound of the solution $h( x ) = ( 1 - \gamma_n ) x$, when $n \geq N$. The lower bound on $R_n$ is obtained by solving $\ell( x ) = ( 1 - \gamma_n ) x$, where $\ell: x \mapsto x - ( 1 / 2 ) x^2$ is a global lower bound on $h$.
%\end{proof}
%
%\begin{rem}
%The constant $3$ in the upper bound is arbitrarily chosen. One may replace it by any constant strictly larger than $2$, with the corresponding necessary modification on the lower bound of $n$.
%\end{rem}
%
%Now we prove the corollary. Since $R_n$ is a monotonically decreasing sequence converging to $0$, when $n$ is large enough, we have $\mathcal{B}_{R_n} \subset \mathcal{N}_{\beta^*}$ for any given $\mathcal{N}_{\beta^*}$. To have the inclusion $\mathcal{B}_{r_n} \subseteq \mathcal{B}_{R_n}$, it suffices to require
%\begin{equation}
%\tau_n \gg \frac{M_n^2}{s M_{n, \beta^*}}, \notag
%\end{equation}
%based on Proposition \ref{prop_ln1+x}.


==> sections/proof_equivalence.tex <==
\begin{prop}
Consider a function $f \in C^3 ( \mathrm{\dom{f}} )$ with domain $\dom{f} \subseteq \mathbb{R}^p$. Fix $x^* \in \dom{f}$, and let $\mathcal{N}_{x^*}$ be an open neighborhood of $x^*$ in $\dom{f}$. Let $K \geq 0$. The following statements are equivalent.

\begin{enumerate}
\item $D^2 f ( x )$ is locally Lipschitz continuous with respect to $x^*$; that is,
\begin{equation}
\norm{ D^2 f ( x^* + \delta ) - D^2 f ( x^* ) }_2 \leq K \norm{ \delta }_2, \label{eq_smooth_D2}
\end{equation}
for any $\delta \in \mathbb{R}^P$ such that $x^* + \delta \in \mathcal{N}_{x^*}$.

\item $D^3 f ( x )$ is locally bounded; that is, 
\begin{equation}
\abs{ D^3 f ( x^* + \delta ) [ u, v, w ] } \leq K \norm{ u }_2 \norm{ v }_2 \norm{ w }_2 \label{eq_smooth_D3}
\end{equation}
for any $\delta \in \mathbb{R}^P$ such that $x^* + \delta \in \mathcal{N}_{x^*}$, and for all $u, v, w \in \mathbb{R}^p$.
\end{enumerate}

\end{prop}

\begin{proof}
Suppose that (\ref{eq_smooth_D2}) holds. By proposition 3.3, it suffices to prove 
\begin{equation}
\abs{ D^3 f ( x^* + \delta ) [ u, u, u ] } \leq K \norm{ u }_2^3 \notag
\end{equation}
for all $u \in \mathbb{R}^p$. By definition,
\begin{align}
\abs{ D^3 f ( x^* + \delta ) [ u, u, u ] }  &= \abs{ \left\langle u, H u \right\rangle } \notag \\
&\leq \norm{ H }_2 \norm{ u }^2, \notag
\end{align}
where
\begin{equation}
H := \lim_{t \to 0} \frac{ D^2 f ( x^* + \delta + t u ) - D^2 f ( x^* + \delta ) }{t}. \notag
\end{equation}
The we have (\ref{eq_smooth_D3}) because $\norm{ H }_2 \leq K \norm{ \delta }_2$ by (\ref{eq_smooth_D2}).

Suppose that (\ref{eq_smooth_D3}) holds. Then we have $\norm{ D^3 f ( x^* + \delta ) [ u ]}_2 \leq K \norm{u}_2$. By the mean value theorem \cite{Zeidler1995},
\begin{align}
D^2 f ( x^* + \delta ) = D^2 f ( x^* ) + \int_0^1 D^3 f ( x_t ) [ \delta ] \, dt, \notag
\end{align}
where $x_t := x^* + t \delta$. Then, by (\ref{eq_smooth_D3}), 
\begin{align}
& \norm{ D^2 f ( x^* + \delta ) - D^2 f ( x^* ) }_2 \notag \\
&\quad = \norm{ \int_0^1 D^3 f ( x_t ) [ \delta ] \, dt }_2 \notag \\
&\quad \leq K \norm{ u }_2. \notag
\end{align}
This completes the proof.

\end{proof}

%We make use of basic properties of Fr\'{e}chet derivatives in this proof. Readers unfamiliar with Fr\'{e}chet derivatives are recommended to find the definitions and properties in standard reference books, such as \cite{Zeidler1986}. 
%
%We point out some notations that might be confusing. The third-order Fr\'{e}chet derivative $D^3 f (x)$ is a $3$-linear symmetric form for any $f \in C^3 ( \dom{f} )$ and $x \in \dom{f}$. We denote the value of $D^3 f (x)$ applied to $u, v, w \in \mathbb{R}^p$ by $D^3 f (x) [u,v,w]$; this coincides with our definition of $D^3 f (x) [ u, u, u ]$ in Section 2 of the paper. $D^3 f (x) [u]$ is a $2$-linear symmetric form, or a symmetric matrix, and $D^3 f( x ) [ u, v, w ] = \left( D^3 f(x) [u] \right) [v, w]$. Then the notation $\norm{ D^3 f (x) [ u ] }_2$ denotes the corresponding spectral norm of $D^3 f (x) [ u ]$. Similarly, $D^2 f(x) [u]$ is a $1$-linear form, or a vector.
%
%Suppose that (\ref{eq_LKC_D2}) holds. By definition, 
%\begin{align}
%\abs{ D^3 L_n ( \beta^* + \delta ) [ u, u, u ] } = \abs{ \left\langle u, H u \right\rangle } \leq \norm{ u }_2 \norm{ H u }_2 , \notag
%\end{align}
%where
%\begin{align}
%H &:= D^3 L_n ( \beta^* + \delta ) [ u ] \notag \\
%&= \lim_{t \to 0} \frac{ D^2 L_n ( \beta^* + \delta + t u ) - D^2 L_n ( \beta^* + \delta ) }{ t }. \notag
%\end{align}
%By definition and (\ref{eq_LKC_D2}), 
%\begin{align}
%& \norm{ H u }_2 \notag \\
%&\quad = \lim_{ t \to 0 } \frac{ \norm{ \left( D^2 L_n ( \beta^* + \delta + t u ) - D^2 L_n ( \beta^* + \delta ) \right) u }_2 }{ t } \notag \\
%&\quad \leq K \norm{ u }_2^2. \notag
%\end{align}
%This implies (\ref{eq_LKC_D3}).
%
%Suppose that (\ref{eq_LKC_D3}) holds. By the mean value theorem, 
%\begin{align}
%& D^2 L_n ( \beta^* + \delta ) [ u ] \notag \\
%&\quad = D^2 L_n ( \beta^* ) [ u ] + \left( \int_0^1 D^3 L_n ( \beta_t ) [ \delta ] \, dt \right)  u , \notag
%\end{align}
%where $\beta_t := \beta^* + t \delta$. Thus it suffices to show
%\begin{equation}
%\norm{ \left( \int_0^1 D^3 L_n ( \beta_t ) [ \delta ] \, dt \right)  u }_2 \leq K \norm{ \delta }_2 \norm{ u }_2, \notag
%\end{equation}
%for any $\delta, u \in \mathbb{R}^p$ such that $\delta_{\mathcal{S}^c} = u_{\mathcal{S}^c} = 0$. For any $3$-linear symmetric form $A$, we have \cite{Nesterov1994}, for any $u \in \mathbb{R}^p$ such that $u_{\mathcal{S}^c} = 0$, 
%\begin{equation}
%\abs{ A [ u, u, u ] } \leq \norm{ u }_2^3, \notag
%\end{equation}
%if and only if for any $u, v, w \in \mathbb{R}^p$ such that $u_{\mathcal{S}^c} = v_{\mathcal{S}^c} = w_{\mathcal{S}^c} = 0$, 
%\begin{equation}
%\abs{ A [ u, v, w ] } \leq \norm{ u }_2 \norm{ v }_2 \norm{w}_2. \notag
%\end{equation}
%Since $D^3 L_n ( \beta_t )$ is a $3$-linear symmetric form, by assumption,
%\begin{equation}
%\abs{ D^3 L_n ( \beta_t ) [ \delta ] [ u, u ] } \leq K \norm{ \delta }_2 \norm{ u }_2^2 \notag
%\end{equation}
%for all $u \in \mathbb{R}^p$ such that $u_{\mathcal{S}^c} = 0$. Therefore, $\norm{ D^3 L_n ( \beta_t ) [\delta] }_2 \leq K \norm{\delta}_2$ in the restricted sense (with respect to $\mathcal{S}$), and
%\begin{equation}
%\norm{ \left( \int_0^1 D^3 L_n ( \beta_t ) [ u ] \, dt \right)  u }_2 \leq K \norm{\delta}_2 \norm{u}_2. \notag
%\end{equation}
%This completes the proof.

==> sections/review.tex <==
As model selection, or selecting the important entries of a high-dimensional parameter based on random observations, is the main motivation of adopting $\ell_1$-regularized $M$-estimators, it is still unclear what conditions ensure the sparsistency of an arbitrarily given $M$-estimator in the sense of Definition \ref{def_sparsistency}.  For the Lasso, or the linear model, there are \cite{Zhao2006} and its sharpened result \cite{Wainwright2009} showing that as long as the irrepresentability condition is satisfied, the Lasso is sparsistent, even with diverging dimensions. There are also some isolated works on specific $M$-estimators for non-linear models \cite{Ravikumar2010,Ravikumar2011}. (I don't want to cite Bach...) But a structured understanding for \emph{a class} of $M$-estimators is still lacking.

It is easy to apply the theoretical framework in \cite{Wainwright2009} for some classes of $M$-estimators. Consider the two smoothness conditions on $L_n$,
\begin{enumerate}
\item \emph{Lipschitz-continuous gradient}: $\left\Vert \nabla L_n( y ) - \nabla L_n( x )  \right\Vert \leq L_g \left\Vert y - x \right\Vert$ with some $L_g \geq 0$, and
\item \emph{Lipschitz-continuous Hessian}: $\left\Vert \nabla^2 L_n( y ) - \nabla^2 L_n( x )  \right\Vert \leq L_H \left\Vert y - x \right\Vert$ with some $L_H \geq 0$,
\end{enumerate}
and the strong convexity condition, $\left\langle \nabla L_n( y ) - \nabla L_n( x ), y - x \right\rangle \geq \mu \left\Vert y - x \right\Vert^2$ with some $\mu > 0$. We show in Section \ref{sec_summary_proof} that, with these common assumptions in optimization theory \cite{Nesterov2004}, it is direct to prove the sparsistency for $L_n$ that possess Lipschitz-continuous gradients/Hessians and are strongly convex. 

There are, however, some important applications with $L_n$ that don't satisfy those conditions. Examples include gamma and Poisson regression problems where the log-likelihood function involves the logarithmic function, and the graphical learning problem where the loss function involves the log-determinant function. 

==> sections/sketch_proof.tex <==
We briefly describe the main idea of the proof. The whole proof is presented in the supplementary material.

It is desirable to have $\hat{\beta}_n = \check{\beta}_n$, since then we have $\mathsf{supp}\, \hat{\beta}_n = \mathrm{supp}\, \check{\beta}_n$. The following lemma based on the primal-dual witness approach \cite{Wainwright2009} provides a sufficient condition.

\begin{lem} \label{lem_PDW}
We have $\hat{\beta}_n = \check{\beta}_n$ if
\begin{equation}
\left\Vert \left[ \nabla L_n( \check{\beta}_n ) \right]_{\mathcal{S}^{\mathrm{C}}} \right\Vert_{\infty} < \tau_n. \notag
\end{equation}
\end{lem}

By Taylor expansion and the optimality condition for $\check{\beta}_n$, we have
\begin{align}
\left[ \nabla L_n( \check{\beta}_n ) \right]_{\mathcal{S}^{\mathrm{C}}} &= - \tau_n \left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}^{\mathrm{C}}, \mathcal{S}} \left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}}^{-1} \check{z}_{\mathcal{S}} \notag \\
&\quad\,\, + \left[ \nabla L( \beta^* ) \right]_{\mathcal{S}^{\mathrm{C}}} - \left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}^{\mathrm{C}}, \mathcal{S}} \left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}}^{-1} \left[ \nabla L_n( \beta^* ) \right]_{\mathcal{S}} \notag \\
&\quad\,\, + ( r_n )_{\mathcal{S}^{\mathrm{C}}} - \left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}^{\mathrm{C}}, \mathcal{S}} \left[ \nabla^2 L_n( \beta^* ) \right]_{\mathcal{S}, \mathcal{S}}^{-1} ( r_n )_{\mathcal{S}} \notag
\end{align}
with some $\check{z} \in \partial \left\Vert \check{\beta}_n \right\Vert_1$. Thus we have $\left\Vert \left[ \nabla L_n( \check{\beta}_n ) \right]_{\mathcal{S}^{\mathrm{C}}} \right\Vert_{\infty} < \tau_n$ if the irrepresentability condition (\ref{eq_irrepresentability}) holds, and
\begin{equation}
\max \left\{ \left\Vert \nabla L_n( \beta^* ) \right\Vert_{\infty}, \left\Vert r_n \right\Vert_{\infty} \right\} \leq \frac{\alpha}{4} \tau_n. \notag
\end{equation}

